Search for $\text{H}\to \text{b}\bar{\text{b}}$ in association with single top quarks as a test of Higgs couplings

The associated production of Higgs boson and single top quark is of particular interest since it is senstive to the relative sign of the Higgs boson coupling to gauge bosons and the Yukawa coupling $y$ to fermions. The presented analysis is setting upper production limits on a model with $y_\text{t}=-1$, which has an enhanced cross section compared to the standard model expectation. For this it focusses on the Higgs boson decaying to a pair of b quarks and uses the full dataset of $pp$ collisions recorded with the CMS detector in 2012. It reports an upper limit on 7.57 times the expected cross section, with an expected sensitivity of 5.14. This translates into the exclusion of associated tHq production with $y_\text{t}=-1$-like characteristics with a cross section smaller than 1.77\,pb.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = smith_joe

default: testpdflatex

testlatex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}
	

testpdflatex:
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg \
              *.inx *.dvi *.toc *.out *~ ~* */*~ */~* spellTmp 


==> tabLimits.tex <==
%\begin{table}[!ht]
%\begin{center}
%\scalebox{0.88}{
%\begin{tabular}{ccc} \hline\hline
% & data-driven \ttbar & MC \ttbar   \\\hline
%expected & 6.09 & 4.78 \\
%observed & 6.68 & 7.25 \\
%\hline\hline
%\end{tabular}
%}
%\end{center}
%\caption{Expected and observed 95\% confidence level upper limits on
%  $\sigma/\sigma_{y_t = -1}$.}
%\label{tab:results}
% \end{table}

% \begin{table}[!ht]
% \begin{center}
% \scalebox{0.88}{
% \begin{tabular}{cccc} \hline\hline
%         & \bf{comb} & 3T    & 4T     \\ \hline
% MC based exp. & \bf{5.22} & 5.97  & 10.55    \\
% MC based obs. & \bf{7.61} & 6.93  & 19.86     \\ 
% \hline
% Data-driven exp. &  \bf{6.32} & 7.66  & 11.40     \\
% Data-driven obs. & \bf{6.91} & 6.19  & 18.04      \\ 
% \hline \hline
% \end{tabular}
% }
% \end{center}
% \caption{Expected and observed 95\% confidence level upper limits on $\sigma/\sigma_{y_t = -%1}$ for both analysis bins and their combination with the MC based and the data-driven approa%ch.}
% \label{tab:results}
% \end{table}
\renewcommand{\arraystretch}{1.5} 
 \begin{table}[!ht]
 \begin{center}
 \scalebox{0.88}{
 \begin{tabular}{ccc} \hline\hline
         & Expected & Observed       \\ \hline
 \textbf{MC-driven} & $\mathbf{5.14^{+2.14}_{-1.44}}$ & $\mathbf{7.57}$ \\
 Data-driven cross-check & $6.24^{+2.26}_{-1.71}$  & 6.95 \\
 \hline \hline
 \end{tabular}
 }
 \end{center}
 \caption{Expected and observed 95\%~confidence level upper limits on $\sigma/\sigma_{y_t = -1}$ for the combination of both analysis bins for the MC-driven and the data-driven approach. For the expected limits also the $+1\,\sigma$ and $-1\,\sigma$ deviations are displayed.}
 \label{tab:results}
 \end{table}


